Fed-CPrompt: Contrastive Prompt for Rehearsal-Free Federated Continual Learning

Federated continual learning (FCL) learns incremental tasks over time from confidential datasets distributed across clients. This paper focuses on rehearsal-free FCL, which has severe forgetting issues when learning new tasks due to the lack of access to historical task data. To address this issue, we propose Fed-CPrompt based on prompt learning techniques to obtain task-specific prompts in a communication-efficient way. Fed-CPrompt introduces two key components, asynchronous prompt learning, and contrastive continual loss, to handle asynchronous task arrival and heterogeneous data distributions in FCL, respectively. Extensive experiments demonstrate the effectiveness of Fed-CPrompt in achieving SOTA rehearsal-free FCL performance.

==> Chapters/Algorithms/algorithm1.tex <==
\begin{algorithm}
\caption{Algorithm 1}\label{alg:cap}
\begin{algorithmic}
\While{Server Executions:}
    \State  Initialize the server by global model parameters $\theta_G$
    \State  for rounds $r = 1, 2, 3, \cdots$
    \State  Participating K clients register with the server.
    \State  Distribute the global model parameters $\theta_G$ with K clients.
    \State  Randomly select J clients from K clients.
    \While{for J clients $j = 1, 2 , 3, \cdots$}
        \State task labels are created using the labels in the batch in $j^{th}$ device.
        \State $\theta_B = \theta_G$
        \State $\theta = \theta_B + \theta_j + \theta_c$
        \State \textbf{function} Continual\_Learning: 
    
    \EndWhile
\EndWhile
\State \textbf{function} Continual\_Learning:
\State $\mathcal{L}$

\end{algorithmic}
\end{algorithm}


==> Chapters/Algorithms/algorithm2.tex <==
\begin{equation}
    f_r^{avg} = AvgPool(f_r(x_p)[0: N L_p, :])
\end{equation}


\textcolor{blue}{Simple setting all the clients get the same task}
\textcolor{blue}{Algorithm from PromptFl\cite{zhao2022reduce}}

\begin{onecolumn}
\begin{algorithm}
\caption{Algorithm 1}\label{alg:cap}
\begin{algorithmic}

\State \textbf{Input}: $C$ clients indexed by $c$, Number of subset clients $L$,  $R$ communication rounds indexed by $r$, local minibatch size $B$, local epochs $E$, learning rate $\eta$, pretrained model , Prompt pool $\mathbf{P}$, Keys $\mathbf{K}$, and tasks $T$
\State \textbf{Server executes}:
\end{algorithmic}

\begin{algorithmic}[1]
    \State  Initialize the pretrained model global model and send it to all clients.
    \State  Randomly initialize prompt parameters $\mathbf{P_{r=1}}$ and keys $\mathbf{K_{r=1}}$. 
    
    \For{$t= \{ 1,\cdots, T\} $}
    \For {$r \in \{1, \cdots, R \}$}
    \State $L \leftarrow$ Select a subset of clients at random
        \For {each client $c \in L$}
        \State Initialize the Prompt pool for each client $\mathbf{P^c_{r,t}}, \mathbf{K^c_{r,t}} \leftarrow \mathbf{P_{r,t}}, \mathbf{K_{r,t}}$
        \State Training on each client $\mathbf{P_{r+1}^{c}}, \mathbf{K_{r+1}^c}, \phi_{r+1}^c\leftarrow ClientUpdate(\mathbf{P_{r}^{c}}, \mathbf{K^c_{r}})$
        \EndFor
    \State  Total number of samples $N_{r} = \sum_{c=1}^{L}n_{c,r}$
    \State Update prompt pool $P_{r+1 } \leftarrow \sum_{c=1}^{L}\frac{n_c}{N_{r}} P_{r+1}^{c}$
    \State Update Keys $K_{r+1} \leftarrow \sum_{c=1}^{L}\frac{n_c}{N_{r}} K_{r+1}^{c}$
    \State Update Classifier $\phi_{r+1} \leftarrow \sum_{c=1}^{L}\frac{n_c}{N_{r,t}} \phi_{r+1}^{c} $
    \EndFor
    \State Update the prompt pool and keys $P_{t+1 } \leftarrow P_{R} $ , \quad$ K_{t+1 } \leftarrow K_{R}$
    \State Expand the classifier head $\phi_{t+1} = \phi_{t} \cup \phi_{R}$
    \EndFor
    \State  \textbf{return} $\theta_{r+1}$

\end{algorithmic}



\end{algorithm}


\begin{algorithm}
\begin{algorithmic}
\State $ClientUpdate(c,P_{r}^{c}, K_{r}^{c}):$ \% Run on client c

\end{algorithmic}
\caption{Client Side }\label{alg:cap}

\begin{algorithmic}[1]
    % \State $\mathcal{B} \leftarrow$ (split $D_t^c$ corresponding to task $t$ into batches of size $B$)
    
        \For{ each local epoch $i \in \{1, \cdots, E\}$}
            \For{batch $b \in \mathcal{B}$}
             \State Initialize batch specific keys and prompts $K_b, P_b = \{\},\{\} $
             \For {$(x,y) \in b $}
             \State Calculate the query $q(x) = f(x)$
             \State Find top-N similar keys $K_x = \arg \min_{\{s_i\}_{i=1}^n  \subseteq [1,M]} \sum_{i=1}^N \gamma(q(x), k_{s_i})$
             \State Select $P_x$ prompts corresponding to $K_x$
             \State Calculate input embedding $x_e = f_e(x)$ 
             \State Prepend top-N prompts $x_p = [P_{s_{1}} ; \cdots; P_{s_{N}}; x_e] $
             \State Calculate sample Loss $\mathcal{L}_x = \mathcal{L}(g_\phi(f_r^{avg}(x_p)),y) + \lambda \sum_{K_x} \gamma(q(x), K_{s_{i}}) $
             \State Update the selected keys and prompts :  $K_b = K_b \cup K_x , P_b = P_b \cup P_x$
             \EndFor
             \State Calculate batch loss $\mathcal{L}_b$ by accumulating $\mathcal{L}_x$ 
             
             \For{ $(K, P)$  in  $(K_b, P_b)$}
             \State Update $K \leftarrow K - \eta \nabla_K{\mathcal{L}_b}$
             \State Update $P \leftarrow P - \eta \nabla_P{\mathcal{L}_b}$
             \EndFor
             \State Update $\phi \leftarrow \phi - \eta \nabla_\phi{\mathcal{L}_b}$
            \EndFor
        \EndFor
    \State  \textbf{return} $K, P , \phi$
\end{algorithmic}

\end{algorithm}

\end{onecolumn}
\twocolumn


==> Chapters/Algorithms/algorithm3_dualprompt.tex <==
\begin{equation}
    f_r^{avg} = AvgPool(f_r(x_p)[0: N L_p, :])
\end{equation}


\textcolor{blue}{Simple setting all the clients get the same task}
\textcolor{blue}{Algorithm from PromptFl\cite{zhao2022reduce}}

\begin{onecolumn}
\begin{algorithm}
\caption{Algorithm 1}\label{alg:cap}
\begin{algorithmic}

\State \textbf{Input}: $C$ clients indexed by $c$, Number of subset clients $L$,  $R$ communication rounds indexed by $r$, local minibatch size $B$, local epochs $E$, learning rate $\eta$, pretrained model , total tasks $T$,E-Prompts $E_p = \{e_t\}_{t=1}^T$, 
task keys $\mathbf{K} = \{k_t\}_{t=1}^T$,
G-Prompt  $\textbf{g}$, 
$\mathbf{start_g}, \mathbf{end_g}, \mathbf{start_e}, \mathbf{end_e}$
\State \textbf{Server executes}:
\end{algorithmic}

\begin{algorithmic}[1]
    \State  Initialize the pretrained model global model and send it to all clients.
    \State  Randomly initialize $\mathbf{g, E, K}$. 
    
    \For{$t= \{ 1,\cdots, T\} $}
    \For {$r \in \{1, \cdots, R \}$}
    \State $L \leftarrow$ Select a subset of clients at random
        \For {each client $c \in L$}
        \State Initialize the Prompt pool for each client $\mathbf{P^c_{r,t}}, \mathbf{K^c_{r,t}} \leftarrow \mathbf{P_{r,t}}, \mathbf{K_{r,t}}$
        \State Training on each client $\mathbf{P_{r+1}^{c}}, \mathbf{K_{r+1}^c}, \phi_{r+1}^c\leftarrow ClientUpdate(\mathbf{P_{r}^{c}}, \mathbf{K^c_{r}})$
        \EndFor
    \State  Total number of samples $N_{r} = \sum_{c=1}^{L}n_{c,r}$
    \State Update prompt pool $P_{r+1 } \leftarrow \sum_{c=1}^{L}\frac{n_c}{N_{r}} P_{r+1}^{c}$
    \State Update Keys $K_{r+1} \leftarrow \sum_{c=1}^{L}\frac{n_c}{N_{r}} K_{r+1}^{c}$
    \State Update Classifier $\phi_{r+1} \leftarrow \sum_{c=1}^{L}\frac{n_c}{N_{r,t}} \phi_{r+1}^{c} $
    \EndFor
    \State Update the prompt pool and keys $P_{t+1 } \leftarrow P_{R} $ , \quad$ K_{t+1 } \leftarrow K_{R}$
    \State Expand the classifier head $\phi_{t+1} = \phi_{t} \cup \phi_{R}$
    \EndFor
    \State  \textbf{return} $\theta_{r+1}$

\end{algorithmic}



\end{algorithm}


\begin{algorithm}
\begin{algorithmic}
\State $ClientUpdate(c,P_{r}^{c}, K_{r}^{c}):$ \% Run on client c

\end{algorithmic}
\caption{Client Side }\label{alg:cap}

\begin{algorithmic}[1]
    % \State $\mathcal{B} \leftarrow$ (split $D_t^c$ corresponding to task $t$ into batches of size $B$)
    
        \For{ each local epoch $i \in \{1, \cdots, E\}$}
            \For{batch $b \in \mathcal{B}$}
             \State Initialize batch specific keys and prompts $K_b, P_b = \{\},\{\} $
             \For {$(x,y) \in b $}
             \State Calculate the query $q(x) = f(x)$
             \State Find top-N similar keys $K_x = \arg \min_{\{s_i\}_{i=1}^n  \subseteq [1,M]} \sum_{i=1}^N \gamma(q(x), k_{s_i})$
             \State Select $P_x$ prompts corresponding to $K_x$
             \State Calculate input embedding $x_e = f_e(x)$ 
             \State Prefix top-N prompts $x_p = [P_{s_{1}} ; \cdots; P_{s_{N}}; x_e] $
             \State Calculate sample Loss $\mathcal{L}_x = \mathcal{L}(g_\phi(f_r^{avg}(x_p)),y) + \lambda \sum_{K_x} \gamma(q(x), K_{s_{i}}) $
             \State Update the selected keys and prompts :  $K_b = K_b \cup K_x , P_b = P_b \cup P_x$
             \EndFor
             \State Calculate batch loss $\mathcal{L}_b$ by accumulating $\mathcal{L}_x$ 
             
             \For{ $(K, P)$  in  $(K_b, P_b)$}
             \State Update $K \leftarrow K - \eta \nabla_K{\mathcal{L}_b}$
             \State Update $P \leftarrow P - \eta \nabla_P{\mathcal{L}_b}$
             \EndFor
             \State Update $\phi \leftarrow \phi - \eta \nabla_\phi{\mathcal{L}_b}$
            \EndFor
        \EndFor
    \State  \textbf{return} $K, P , \phi$
\end{algorithmic}

\end{algorithm}

\end{onecolumn}
\twocolumn


==> Chapters/Section3/problemstatement.tex <==
\subsection{Problem Statement}
% Define the problem formulation in federated settings
Consider the conventional federated learning scenario with a global server $S_G$ and $K$ clients. 
For each round of training, the server communicates a copy of  the global model to each participating client for local training. 
Each participating client $k \in \{1,2,\cdots K\}$ trains the model on its private data $\mathcal{D}_k\in  \{x_{ki}, y_{ki}\}_{i=k}^{N_t}$ , where $N_t$ is the total number samples at $k$-th client . Each client then transfers its locally learned knowledge to the server $S_G$. 
The servers aggregate the model and distribute the model to the local clients for the next round of training. 

% define federated class incremental setting.
Extending this to  federated class incremental learning tackles a more challenging problem for learning$\mathcal{T_k} \in \{\mathcal{T_k}^t\}_{t=1}^T $, where $T$ is the total number of disjoint incremental tasks at the $k \in \{i\}_0^K$  client.
% Each client k consists of private disjoint incremental tasks $\mathcal{T_k} \in \{\mathcal{T_k}^t\}_{t=1}^T $. 
Further, each classification task at time $t$ at $k$-th client is defined $T_k^t \in  \{x_{ki}^t, y_{ki}^t\}_{t=k}^{N_t}$ , $N_t$ is the number of pairs of unbalanced non-iid data samples. 
At round $r$, The global server $S_G$ communicates the frozen pretrained model and the latest learnable prompts $P_n$  to each new participating client. Each new client $k$ stores the global frozen model, which is reused during training, testing and inference. Further, the client $k$ trains the prompt parameters and the classifier head on the current task $\mathcal{T_k^t}$ and transfers this knowledge to the server $S_G$ for aggregation. The server uses FedAvg \cite{mcmahan2017communication} aggregates the prompts and classifiers head and transfers the updated prompts and classifier head for the next round of training. This process is repeated for $R$ federated training rounds to then transition to task $\mathcal{T_k^{t+1}}$. 
Client $k$ updates the learnable prompt parameters and classifier head. Each client then sends their local updated prompts and classifier parameters to the global server for aggregation. The aggregates the prompts and classifier for the next round of training.  The objective of prompt based federated continual learning is to learn additional lightweight  learnable parameters to  reuse the frozen model while reducing catastrophic forgetting. 

To reuse the existing frozen model like ViT \cite{dosovitskiy2020image} for each incremental task, we use learnable prompts \cite{jia2022visual} to provide additional task information. These prompts conditionally downstream the model to achieve high accuracy without explicitly training the entire model.  


% Consider a global server $S_G$, and $K$ clients each with class incremental tasks. The client $k \in \{1,2,\cdots K\}$ has a set of private incremental tasks $\mathcal{T}_k \in \{\mathcal{T}_k^t,\}_{t=1}^T $, where $T$ is the total number of tasks. A $t$-th task at client $ k$ is defined as $\mathcal{T}_k^t \in \{x_k^t, y_k^t\}_{t=k}^{N_t}$ , where $N_k^t$ are the pairs of data samples, $x_k^t$ is the input space, and $y_k^t \in \mathcal{Y}^t$ are the output labels. $C^t$ is a set of new classes and

% The client aims to learn to predict new classes $C^t$ without reducing its performance on $C^p$. We assume that there are overlapping old and new classes across the clients.  
% At each round $r \in \{1,2,3,\cdots,R\}$, server $S_G$ randomly selects $L \in K$ clients and client $l \in L$ gets the the global server model $\theta^r$ and locally trains on task $T_l^i$ to produce a model $\theta_{l,r}^i$.
% At the end of the synchronous round $r$, the global server aggregates this model such that, $\theta_{r+1} = \frac{1}{|L|}\sum_{l=1}^L \theta_{l,r}^i $. 
% Although the global aggregation is intuitive, this simple aggregation strategy can result in diverged weights when the number of classes on tasks is not equal among clients. More importantly,  there can be catastrophic forgetting on the old server model when new classes are learned. Additionally, the client must also avoid forgetting past tasks while learning new tasks. 
% Inspired by the results in ~\cite{smith2022closer}, we use PredKD+L2(BCE) to learn the new classes while preserving semantic similarity with the previous classes. Finally, to update the model for the next round $r+1$, we use FeatKD to regularize the model update with the past model. 

\textbf{Client loss function}:

\blue{Client-side computation should be rehearsal free.
}

The Cross entropy loss $CE$ for the $k$-th client at round $r$ is defined as,
\begin{equation}\label{eq:PredKDclient}
    \mathcal{L}_{k} = BCE(P_{\theta_{k,r}^t}(x), P_{\theta_{k,r}^{t-1}}(x))
\end{equation}
where $P_{\theta_{k,r}^t}(x)$ is the prediction from local model $\theta_{k,r}^t$ on input feature $x$ for task $t$, and the $P_{\theta_{k,r}^{t-1}}$ are the predictions on the local model at previous task. 

\textbf{Server-side loss function}:

The limitation of rehearsal-based methods is that it is computationally expensive or requires large memory; however, these constraints do not apply to the server. However, rehearsals cannot be directly transferred due to privacy concerns. 
We can have a pretrained public dataset. Since the forgetting happens in the latter layers, we regularize the changes in the former layers using FeatKD and this dataset.
\begin{equation}\label{eq:FeatKDserver}
\mathcal{L}_{FKD} = || \theta_r^l(x) -  \theta_{r-1}^l(x)||^2_2,    
\end{equation}



==> Chapters/experiments.tex <==
\subsection{Experimental Setup}
We consider Cifar-100 split into $T =10$ incremental tasks. Each client receives a subset of data from each task following iid(, and non-iid distribution described later in this section).
We consider total ${K} = 10$ clients, train at their local data. We use a ViT model (ViT\_base\_patch16\_224) pretrained on Imagenet-21k. Additionally, learning rate = 5e-5 or {0.00005, 0.00001, 0.0005, 0.0001} with \textit{Adam} optimizer and batch size of 256. 
After $R1$ rounds $K_1 = 1$ random client(s) move to the subsequent task and train along with the other clients still at the current task. ( We can consider that the $K_1$ client(s) move to the subsequent task when the training accuracy or loss reaches a certain amount e.g. acc = 70 ).
Next, the other clients join on task.

After $R_1 \in R$ rounds $K_1 = 1, K_2 =1$ random client(s) move to the subsequent task $t+1, t+2$, and train along with the other clients still at the current task. ( We can consider that the $K_1$ client(s) move to the subsequent task when the training accuracy or loss reaches a certain amount e.g. acc = 70 ).
Next, the other clients join on task.

During each tasks, prefix prompts are added to the layers 1-5 of the ViT network of prompt length {5, 8, 10, 20} and 100 prompts(10 per task). 

\subsection{Implementation Details}
We use the following two datasets to test the effectivness of our approach: CIFAR-100, 5-Datasets (SVHN, FashionMNIST, MNIST, NOTMNIST, CIFAR-10) and \rule{1cm}{0.15mm} for comprehensive comparison. We utilize the ViT network pretrained on the Imagenet dataset as the classification model. We divide each dataset into 10 non-overlapping tasks. Additionally, to train the prompt parameters, the learning rate is $0.003$ and employ an Adam optimizer. We train for 30 global rounds and 3 local epochs. We select all the local clients to train for each global round.
% We randomly select $10\%$ clients in each round.

Following the prompt-based learning in \cite{wang2022learning}, we freeze the pretrained ViT network and add a trainable prompt pool and classification (MLP) head to the network. The prompt pool consists of 10 prompts, each of length 10, and select top 5 prompts from the pool. After each round of training, the weights are aggregated following the FedAvg algorithm \cite{mcmahan2017communication}. 

Additionally, we compare the performance of the models on iid and different non-iid settings. For iid,  each client has uniformly distributed data of the current task. Therefore at each task, the each client out of 10 clients, will have 500 uniformly distributed data samples. However, for non-iid settings, the data samples are distributed according to distribution based label imbalance, where each client will have data samples based on Dirichlet distribution with $\beta = 0.1$.

In order to test the performance of various loss functions attach the task invariant prompts at locations $1\rightarrow3$  and task specific prompts at $4\rightarrow 8$. We compare the testing accuracy in Federated class incremental settings for conventional cross entropy loss, binary cross entropy, and binary cross entropy (BCE) with gradient compensation (BCE + GC).



\subsection{Results}


% \begin{table*}[!tbh]
% \caption{CIFAR-100, 10 clients , iid}
% \begin{adjustbox}{width =1\textwidth}

% \begin{tabular}{|c|ccccccccccc|}
% \hline
% \multirow{2}{*}{Model} &
%   \multicolumn{11}{c|}{Accuracy | forgetting} \\ \cline{2-12} 
%  &
%   \multicolumn{1}{c|}{task 1} &
%   \multicolumn{1}{c|}{task 2} &
%   \multicolumn{1}{c|}{task 3} &
%   \multicolumn{1}{c|}{task 4} &
%   \multicolumn{1}{c|}{task 5} &
%   \multicolumn{1}{c|}{task 6} &
%   \multicolumn{1}{c|}{task 7} &
%   \multicolumn{1}{c|}{task 8} &
%   \multicolumn{1}{c|}{task 9} &
%   \multicolumn{1}{c|}{task 10} &
%   Average Accuracy \\ \hline
% Upper Bound &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%    \\ \hline
% Fed-FT &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%    \\ \hline
% Fed-EWC &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%    \\ \hline
% Fed-LwF &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%    \\ \hline
% Fed-DualPrompt &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%    \\ \hline
% Fed-CODAPrompt &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%    \\ \hline
% \end{tabular}
% \end{adjustbox}
% \end{table*}
% We use the conventional federated learning without continual learning as the upperbound and compare it with iid and non-iid settings.
% \textbf{Iid data}  

\textbf{Performance Comparison of the proposed method with baselines:}
To illustrate the effectiveness of our framework, we compare the following approaches.
\textbf{FedEWC} \cite{shoham2019overcoming} denotes a rehearsal free methods with EWC \cite{kirkpatrick2017overcoming}. \textbf{FedLwf-2}\cite{usmanova2022federated} is a rehearsal-free knowledge distillation method with FedAvg with two teachers. \textbf{CFed}\cite{ma2022continual} is a knowledge distillation method in addition uses a surrogate data. We measure the performance using the average accuracy and forgetting on the on the previous tasks.

Done
SynIID, FedCODA, FedDual, Fed-L2P, Fed-LwF
AsynIID, FedCODA, FedDual, Fed-L2P, Fed-LwF (551)

SynNonIID, FedCODA, FedDual, Fed-L2P
AsynNonIID, FedCODA, FedDual (551)
SynIID Ours
SynNonIID Ours

Running
AsynIID, Ours (551), 
AsynNonIID, Ours (551),
ours (552), FedCODA (552)

Waiting
Ours Ablation: no triple, (SynIID, SynNonIID)
% Ours: 1 triple loss (noniid, forgetting)


(FedCODA, FedDual), 10 clients
1) Syn IID, Fed-EWC, Fed-LwF, Fed-L2P
2) Asy IID, Fed-EWC, Fed-LwF, Fed-L2P, (5,5;1)
3) Syn NonIID, Label Skew, $\beta=0.5$
4) Asy NonIID, Label Skew, $\beta=0.5$
5) Syn NonIID, Label Skew, $\beta=0.5$, regularization (key, whole model, FedCODA)

0) Asy, (5,5;2) Asy, (3,3,4;1) (3,3,4;2)
1) new datasets, new tasks
2) NonIID, label skew, $\beta=0.1, 0.01$; quantity skew, $\beta=0.5, 0.1$


% Please add the following required packages to your document preamble:
% \usepackage{multirow}


% \begin{table*}[!tbh]

% \begin{adjustbox}{width =1\textwidth}
% \begin{tabular}{|c|ccccccccccc|}
% \hline
% \multirow{2}{*}{Model} &
%   \multicolumn{11}{c|}{Accuracy | forgetting} \\ \cline{2-12} 
%  &
%   \multicolumn{1}{c|}{task 1} &
%   \multicolumn{1}{c|}{task 2} &
%   \multicolumn{1}{c|}{task 3} &
%   \multicolumn{1}{c|}{task 4} &
%   \multicolumn{1}{c|}{task 5} &
%   \multicolumn{1}{c|}{task 6} &
%   \multicolumn{1}{c|}{task 7} &
%   \multicolumn{1}{c|}{task 8} &
%   \multicolumn{1}{c|}{task 9} &
%   \multicolumn{1}{c|}{task 10} &
%   Average Accuracy \\ \hline
% ViT (fine tuning) &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%    \\ \hline
% ViT() upperbound &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%    \\ \hline
% ViT(EWC) &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%    \\ \hline
% ViT(LwF) &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%    \\ \hline
% Vit(ours) &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%    \\ \hline
% \end{tabular}
% \end{adjustbox}
% \end{table*}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}
\centering
\caption{Model performance}
\label{tab:models}
\begin{tabular}{@{}llcc@{}}
\toprule
\multicolumn{2}{c}{Model} & Accuracy & Forgetting \\
\cmidrule(lr){1-2}\cmidrule(lr){3-4}
\multicolumn{2}{c}{Upper Bound} & & \\
\midrule
\multirow{5}{*}{Sync - IID} & Fed-EWC & 9.79 & 84.85 \\
& Fed-LwF & 60.92 & 33.75 \\
& Fed-L2P & 73.19 & 9.8 \\
& Fed-DualPrompt & 76.00 & 9.84 \\
& Fed-CODAPrompt & 77.28 & 6.42 \\
\midrule
\multirow{3}{*}{\shortstack[l]{Sync NIID \\ $(\beta = 0.5)$\\ Label Skew}}
& Fed-L2P &   & \\
& Fed-DualPrompt & 46.28 & 13.16 \\
& Fed-CODAPrompt & 54.8 & 11.55\\
\midrule
\multirow{3}{*}{\shortstack[l]{Sync NIID \\ $(\beta = 0.1)$\\ Quantity Skew}}
& Fed-L2P &  & \\
& Fed-DualPrompt & 77.57 & 8.38 \\
& Fed-CODAPrompt & 78.56 & 5.00 \\
\midrule
\multirow{5}{*}{Asynchronous IID} 
& Fed-EWC & & \\
& Fed-LwF & 37.70 & 53.68\\
& Fed-L2P & 69.95 & 14.39 \\
& Fed-DualPrompt & 70.27 & 17.36 \\
& Fed-CODAPrompt & 73.63 & 10.94 \\
\midrule
\multirow{3}{*}{\shortstack[l]{Asynchronous NIID \\ $(\beta = 0.5)$\\ Label Skew}} 
& Fed-L2P & & \\
& Fed-DualPrompt & 37.12 & 6.98\\
& Fed-CODAPrompt & 51/23 & 9.03 \\
\bottomrule
\end{tabular}
\end{table}


\textbf{Effectiveness of our loss function} We test 3 types of loss functions, the conventional cross-entropy loss used for classification. Additionally, we test binary cross entropy (BCE) to address the class imbalance among clients. We compare the performance of CE and BCE function with the modified gradient compensation loss proposed by \cite{dong2022federated}. BCE loss functions provides considerable improvements over CE to prevent forgetting as shown in Fig ~\ref{fig:compare_lf}.



\begin{figure}[!tb]
\centerline{\includegraphics[width=0.5\textwidth]{Figures/lossfunction.png}}
\caption{Test accuracy while training in class incremental setting with prompts on cross entropy loss function, binary cross entropy (BCE) and BCE with gradient compensation(GC)  }
\label{fig:compare_lf}
\vspace{-1em}
\end{figure}




% \begin{table}[tbh]
% \begin{tabular}{|c|c|c|}
% \hline
% Loss type      & Average Accuracy & Forgetting \\ \hline
% ViT (CE)       &     50.88      &   33.41      \\ \hline
% ViT (BCE)      &     71.62      &   2.83         \\ \hline
% ViT (BCE + GC) &     71.28      &   3.73         \\ \hline
% \end{tabular}
% \caption{Accuracy and Forgetting of when using Cross-entropy loss, binary-cross entropy and graient compensation(GC) with BCE. }
% \label{tab:losscomparision}
% \end{table}




\textbf{How to attach the prompts:} Prompts were originally designed to store task-spefic information. However, we need to task-invariant prompts to transfer knowledge among tasks. We test that two types of prompts are required by comparing the performance of task-specific prompts with combination of task-specific and task-invariant prompts.



\textbf{Where to attach the prompts:} We choose the ViT-B models with 12 layers in total. To test where to attach the both task-invariant and task specific prompts only to the input embedding to the first transformer layer. Next, the two prompts to all the two layers of ViT's input embedding. Based on this observation, we attach the prompts to 1-6 layers and 7-12 layers. We observe that the performance drops when we attach the prompts to the deeper layers. 



% \textbf{Effectiveness of  prompt:} 
 From Table \ref{tab:promptlocation}, we observe that the prompt are more effective when applied to the shallow layers of the ViT network. We, therefore, attach task invariant prompts at 1-3 and test task-specific prompts at 1-3, 3-5, and 4-6. Then we attach the task-specific prompts at 4-6, and test the task-invariant prompts at 1-3, 3-5, 4-6.
 
 \begin{figure}[!tb]
\centerline{\includegraphics[width=0.5\textwidth]{Figures/promptlocations.png}}
\caption{Test accuracy while training in class incremental setting with prompts at location $1\rightarrow12, 1\rightarrow6 , 7\rightarrow12$ and $1$.}
\label{fig:compare_lf}
\vspace{-1em}
\end{figure}

 

% \begin{table}[tbh] 
% \begin{tabular}{|c|c|c|}
% \hline
% Prompt location & Total accuracy & Forgetting \\ \hline
% 1                              &   69.13        &    1.66    \\ \hline
% 1-12                           &   66.2             &            \\ \hline
% 1-6                            &   72.04        &    4.27    \\ \hline
% 7-12                           &   56.10        &    7.98   \\ \hline
% 1-3                            &  training started               &            \\ \hline
% 4-6                            & training started                &            \\ \hline
% 7-9                            &training started                 &            \\ \hline
% 10-12                          & training started                &            \\ \hline
% \end{tabular}
% \caption{Accuracy and Forgetting of prompts at different prompt configurations }
% \label{tab:promptlocation}
% \end{table}

\textbf{Scalability} We show that our prompt-based approach is scalable, we test with 50 clients with cifar-100 data, and 100 clients with 5-datasets.  






% \begin{table}[tbh] 
% \begin{tabular}{|c|c|c|}
% \hline
% Task invariant prompt location & Total accuracy & Forgetting \\ \hline
% 1-12                           &                &            \\ \hline
% 1                              &                &            \\ \hline
% 1-6                            &                &            \\ \hline
% 7-12                           &                &            \\ \hline
% 1-3                            &                &            \\ \hline
% 4-6                            &                &            \\ \hline
% 7-9                            &                &            \\ \hline
% 10-12                          &                &            \\ \hline
% \end{tabular}
% \caption{Accuracy and Forgetting of prompts at different task-invariant configurations }
% \label{tab:taskinvP}
% \end{table}



% \begin{table}[tbh] 
% \begin{tabular}{|c|c|c|}
% \hline
% Initialization type & Total accuracy & Forgetting \\ \hline
% Random initialization                 &                &            \\ \hline
% Last task                            &                &            \\ \hline
% Average of previous prompts          &                &            \\ \hline
% similarity based selection           &                &            \\ \hline

% \end{tabular}
% \caption{Task-specific prompt initialization}
% \label{tab:prompt initialization}
% \end{table}




\begin{table}[]
\begin{tabular}{|cc|c|c|}
\hline
\multicolumn{2}{|c|}{Model}                                           & Test accuracy (\%) & Forgetting \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{L2P}}         & iid              &    78.73           &   7.31         \\ \cline{2-4} 
\multicolumn{1}{|c|}{}                             & non iid beta 0.1 &  70.67          &   9.61  \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Dual Prompt}} & iid              &     82.01            &      5.86      \\ \cline{2-4} 
\multicolumn{1}{|c|}{}                             & non iid beta 0.1 & 82.44         &  3.22     \\ \hline

\end{tabular}
\end{table}

\begin{figure}[!tb]
\centerline{\includegraphics[width=0.4\textwidth]{Figures/Test_Accuracy.png}}
\caption{Testing accuracy for learning to prompt (L2P) and Dual Prompt under IID and Non IID respectively ($\beta = 0.1$).}
\label{fig:trainingleModality}
\vspace{-1em}
\end{figure}

\subsection{Ablation Studies}
As shown in Table \blue{table}, we investigate the effects of type of prompts in the Federated Class incremental setting. Our-w/oTS and Ours-w/oTI denote the performance of our model without using task-specific and task invariant prompts respectively.









% \begin{algorithm}
% \caption{Algorithm 1}\label{alg:cap}
% \begin{algorithmic}
% \Require $n \geq 0$
% \Ensure $y = x^n$
% \State $y \gets 1$
% \State $X \gets x$
% \State $N \gets n$
% \While{$N \neq 0$}
% \If{$N$ is even}
%     \State $X \gets X \times X$
%     \State $N \gets \frac{N}{2}$  \Comment{This is a comment}
% \ElsIf{$N$ is odd}
%     \State $y \gets y \times X$
%     \State $N \gets N - 1$
% \EndIf
% \EndWhile
% \end{algorithmic}
% \end{algorithm}



==> Chapters/plan.tex <==
To check the where to attach the task-specific prompts we empirically analyze different positions to attach the prompts in Table \ref{tab:taskinvP}. First, we add the task-specific prompts to 1-12 layers of the ViT network. Next, we test only adding task-specific prompt to the first embedding layer. Further, we test adding prompts to the 1-6 and 7-12 layers, i.e. the first and last 6 layers of the ViT network respectively. Finally,  we test 1-3,4-6,7-9, 10-12 settings to closely observer the effects of position of prompts on the forgetting. For all these experiments the task-invariant prompts are attached to the 1-3 layers of the ViT network.


Similarly, we test the task-invariant prompt location in Table \ref{tab:taskinvP}.

To address the class imbalance among clients we consider binary-cross entropy(BCE) loss. We compare the results with conventional cross-entropy loss and class-aware gradient compensation loss ~\cite{dong2022federated} in Table \ref{tab:losscomparision}. 


\textbf{Task specific prompt initialization} There can be many ways to initialize the task-specific prompts. We compare, randomly initializing prompts for each task, selecting the tuned prompt from the last task, taking the average of the all the previous prompts, and similarity based selection from the previous task-specific prompts. We test the accuracy after \blue{10} rounds of training.







\begin{enumerate}
    \item Create a fed continual learning dataset. 
    \item  Create a custom Fed Learning algorithm. 
    \item Verify the algorithm
    \item add random seed to recreate the experiments
    \item Analyze the parameters

\end{enumerate}
\textbf{Datasets}
\begin{itemize}
    \item CIFAR-100
    \item 5-datasets (class-incremental) (SVHN + FASHION MNIST , MNIST, NOTMNIST, CIFAR-10)
    \item Split ImageNet-R. (probably)
    \item else  use TinyImageNet. or Caltech-256
\end{itemize} 

\begin{enumerate}
    \item Comparison methods 
    \begin{itemize}
        \item FCIL ( for rehearsal based comparision)
        \item iCaRL + FL 
        \item FedEWC
        \item FedLwf
        \item CFed (second paper)
        
    \end{itemize}
\end{enumerate}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table}[]
% \begin{tabular}{|cc|c|c|}
% \hline
% \multicolumn{2}{|c|}{Experiment}                                                                                                                                                               & Cifar 100 dataset     & 5 datasets            \\ \hline
% \multicolumn{1}{|c|}{\multirow{3}{*}{loss}}                                                                 & cross-entropy                                                                    & training started      &                       \\ \cline{2-4} 
% \multicolumn{1}{|c|}{}                                                                                      & \begin{tabular}[c]{@{}c@{}}binary cross\\ entropy(BCE)\end{tabular}              & training started      &                       \\ \cline{2-4} 
% \multicolumn{1}{|c|}{}                                                                                      & BCE + GC                                                                         & training started      &                       \\ \hline
% \multicolumn{1}{|c|}{\multirow{8}{*}{prompt position}}                                                      & 1                                                                                &  53.54 (14.34)                     &                       \\ \cline{2-4} 
% \multicolumn{1}{|c|}{}                                                                                      & 1-12                                                                             &   55.65 (15.51)                    &                       \\ \cline{2-4} 
% \multicolumn{1}{|c|}{}                                                                                      & 6-12                                                                             &                       &                       \\ \cline{2-4} 
% \multicolumn{1}{|c|}{}                                                                                      & 7-12                                                                             &                       &                       \\ \cline{2-4} 
% \multicolumn{1}{|c|}{}                                                                                      & 1-3                                                                              &                       &                       \\ \cline{2-4} 
% \multicolumn{1}{|c|}{}                                                                                      & 4- 7                                                                             &                       &                       \\ \cline{2-4} 
% \multicolumn{1}{|c|}{}                                                                                      & 7-9                                                                              &                       &                       \\ \cline{2-4} 
% \multicolumn{1}{|c|}{}                                                                                      & 10-12                                                                            &                       &                       \\ \hline
% \multicolumn{1}{|c|}{\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Baselines \\ Continual learning\end{tabular}}} & FCL-Fine tuning                                                                  &                       &                       \\ \cline{2-4} 
% \multicolumn{1}{|c|}{}                                                                                      & \multicolumn{1}{l|}{ViT- EWC}                                                    &  \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\ \cline{2-4} 
% \multicolumn{1}{|c|}{}                                                                                      & \multicolumn{1}{l|}{ViT-LwF}                                                     & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\ \cline{2-4} 
% \multicolumn{1}{|c|}{}                                                                                      & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}ViT- Ours\\ Prompts\end{tabular}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\ \hline
% \end{tabular}
% \end{table}


==> Chapters/proposedmethod.tex <==
In Section \ref{sec:promptmechanism} we introduce how to attach the prompts to a single multi-head self-attention (MSA) layer. Finally, inspired from \cite{wang2022learning}, we adapt a prompt selection mechanism to effectively select e-prompts.

\subsection{Prompt Mechanism}\label{sec:promptmechanism}



\subsection{task specific-prompt selection mechanism}

